Space-Efficient Latent Contracts

Standard higher-order contract monitoring breaks tail recursion and leads to space leaks that can change a program's asymptotic complexity; space-efficiency restores tail recursion and bounds the amount of space used by contracts. Space-efficient contract monitoring for contracts enforcing simple type disciplines (a/k/a gradual typing) is well studied. Prior work establishes a space-efficient semantics for manifest contracts without dependency (Greenberg 2015); we adapt that work to a latent calculus with dependency. We guarantee space efficiency when no dependency is used; we cannot generally guarantee space efficiency when dependency is used, but instead offer a framework for making such programs space efficient on a case-by-case basis.

==> texdirectives.tex <==
\fulltrue

